Arriving on time: estimating travel time distributions on large-scale road networks

Most optimal routing problems focus on minimizing travel time or distance traveled. Oftentimes, a more useful objective is to maximize the probability of on-time arrival, which requires statistical distributions of travel times, rather than just mean values. We propose a method to estimate travel time distributions on large-scale road networks, using probe vehicle data collected from GPS. We present a framework that works with large input of data, and scales linearly with the size of the network. Leveraging the planar topology of the graph, the method computes efficiently the time correlations between neighboring streets. First, raw probe vehicle traces are compressed into pairs of travel times and number of stops for each traversed road segment using a `stop-and-go' algorithm developed for this work. The compressed data is then used as input for training a path travel time model, which couples a Markov model along with a Gaussian Markov random field. Finally, scalable inference algorithms are developed for obtaining path travel time distributions from the composite MM-GMRF model. We illustrate the accuracy and scalability of our model on a 505,000 road link network spanning the San Francisco Bay Area.

==> modelling.tex <==
%!TEX root =article.tex
We combine 3 different graphs

The road network is described as a set of $n$ directed links $l_{i}$.
Each link $l\in\mathcal{L}$

The travel time on each link is a multimodal Gaussian distribution:
a mixture of $m_{l}$ modes. Each of the modes is indexed by some
random variable $S_{l}$ and the set of all modes is $\mathcal{S}_{l}$
for link $l$. The travel time that corresponds to mode $s_{l}$ of
link $l$ is represented by a random variable $Y_{l,s_{l}}$. Thus
the travel time on one link is:
\[
TT_{l}=\sum_{s\in\mathcal{S}_{/}}\mathbf{1}_{s}\left(S_{l}\right)Y_{l,s}
\]


All the random variables $\left(Y_{l,s}\right)_{l\in\mathcal{L},s\in\mathcal{S}_{l}}$
can be stacked into a single vector of size $m=\sum_{l}m_{l}$.
\[
Y_{a,\text{Red}}
\]
\jdrcomment{ what is this? $Y_{a,\text{Red}}$}

Observation and pipeline:

$Y_{l,s}$ is the travel time on link $l$ when state $s$ is activated,
with $s\in\mathcal{S}_{l}$. This travel time is a Gaussian random
variable with mean $\mu_{l,s}$ and variance $\sigma_{l,s}$. The
vector $Y=\left(Y_{l,s}\right)_{l\in\mathcal{L},s\in\mathcal{S}_{l}}$is Gaussian:

\[
Y\sim\mathcal{N}\left(\mu,\Sigma\right)
\]


The $\beta$ function gives the mapping between the variables and
the link and state. 
\[
\beta\left(l,s\right)
\]
\[
\beta\,:\,\cup_{l}\left\{ l\right\} \times\mathcal{S}_{l}\rightarrow\mathbb{N}
\]


Pipeline:

An observed trajectory is a sequence of timestamped lat/longs coordinates
that pertain to one vehicle. The observations are map-matched. An
observed trajectory is then a sequence of timestamped locations on
the road graph:
\[
\left(t_{j},l_{j},o_{j}\right)_{j=0\cdots J}
\]


From this sequence of locations, one can infer the behavior of the
vehicle: where it stopped, where it had a green light. This step of
trajectory decomposition leads to a representation of the trajectory
as a sequence of states and variables:
\[
\left(l_{1},G,t_{1}\right)\,\,\left(l_{2},R,t_{2}\right)\,\,\left(l_{3},G,t_{3}\right)\,\,\cdots\left(l_{M},G,t_{M}\right)
\]
\[
z=\left(l_{i},s_{i},y_{l_{i},s_{i}}\right)_{i=1\cdots M}
\]


We simplify the representation of the observation into a vector form:
\[
z=\left(\hat{y},P\right)
\]
 with $P\in\mathbb{R}^{M\times N}$ with $P_{i\beta\left(l_{i},s_{i}\right)}=1$
and $0$ everywhere else. (We neglect for now the case of duplicate
links)
\[
\hat{y}\sim\mathcal{N}\left(P\mu,P\Sigma P^{T}\right)
\]
\[
\log\pi\left(z\right)=\cdots-\frac{1}{2}\log\left|P\Sigma P^{T}\right|-\frac{1}{2}\left(\hat{y}-P\mu\right)^{T}\left(P\Sigma P^{T}\right)^{-1}\left(\hat{y}-P\mu\right)
\]


\[
\mathcal{L}=\sum_{u}\log\pi\left(z^{\left(u\right)}\right)
\]


This expression is, as far as we know, not convex and may have multiple
local minima. Two strategies are possible:

Data completion, in which the vector is completed. This is the EM
algorithm.

Simplify the problem by building some sufficient statistics.

Consider the simpler scenario in which all the empirical covariance
matrix $\tilde{\Sigma}$ is observed. The maximum likelihood problem
to find the empirical covariance matrix is:

\jdrcomment{do you mean to find the precision matrix?}
\[
\text{minimize}\,\,-\log\left|S\right|+\text{Tr}\left(S\tilde{\Sigma}\right)
\]
\[
S_{uv}=0\,\,\forall\,\left(u,v\right)\notin\mathcal{E}
\]


Observation: this problem only depends on $m$ terms of the covariance
matrix! 
\[
\text{Tr}\left(S\tilde{\Sigma}\right)=\sum_{\left(u,v\right)\in\mathcal{E}}S_{uv}\tilde{\Sigma}_{uv}
\]


Instead of considering the individual likelihoods of each observation
individually, we consider the covariance that would be produced if
each observation was aggregated at into a single covariance matrix.
This approach discards some information, however if the elements were
uniformly sampled. it should give the same result.

\jdrcomment{previously, the $i$ index was used to iterate along a path, I don't see how indexing $i$ makes sense in this aggregation calculation.}

\[
N_{i}=\text{card}\left(\left\{ p\,:\,\exists u\,:\, P_{u\beta\left(l_{i},s_{i}\right)}^{\left(p\right)}=1\right\} \right)
\]
\[
\mathbb{E}_{i}\left[f\left(Y_{i}\right)\right]=\frac{1}{N_{i}}\sum_{p}\sum_{u\,:\, P_{u\beta\left(l_{i},s_{i}\right)}^{\left(p\right)}=1}f\left(\hat{y}_{u}^{\left(p\right)}\right)
\]


Similarly, we are going to define the second order terms for the observations
that span 2 states:
\[
N_{i\cap j}=\text{card}\left(\left\{ p\,:\,\exists u,v\,:\, P_{u\beta\left(l_{i},s_{i}\right)}^{\left(p\right)}=1\,\text{and }P_{v\beta\left(l_{j},s_{j}\right)}^{\left(p\right)}=1\right\} \right)
\]
\[
\mathbb{E}_{i\cap j}\left[f\left(Y_{i},Y_{j}\right)\right]=\frac{1}{N_{i\cap j}}\sum_{p}\sum_{u,v\,:\,\begin{array}{c}
P_{u\beta\left(l_{i},s_{i}\right)}^{\left(p\right)}=1\\
P_{v\beta\left(l_{j},s_{j}\right)}^{\left(p\right)}=1
\end{array}}f\left(\hat{y}_{u}^{\left(p\right)},\hat{y}_{v}^{\left(p\right)}\right)
\]


Empirical covariance vector:
\[
\hat{\mu}_{i}=\mathbb{E}_{i}\left[Y_{i}\right]
\]


Call $\hat{\Sigma}$ the partial empirical covariance matrix:
\[
\hat{\Sigma}_{ij}=\begin{cases}
\mathbb{E}_{i\cap j}\left[Y_{i}Y_{j}\right]-\mathbb{E}_{i}\left[Y_{i}\right]\mathbb{E}_{j}\left[Y_{j}\right] & \text{if }N_{ij}>0\\
0 & \text{otherwise}
\end{cases}
\]


Using this PECM as a proxy for the real covariance matrix, one can
then estimate the most likely GMRF by solving the following problem:
\[
\min\,\,-\log\left|S\right|+\left\langle S,\hat{\Sigma}\right\rangle 
\]


If $\hat{\Sigma}$ is positive definite, this problem is convex and
has a unique solution. Note in particular that $\hat{\Sigma}$ is
not necessarily positive semi-definite, since in particular:
\[
\mathbb{E}_{i\cap j}\left[Y_{i}^{2}\right]\neq\mathbb{E}_{i}\left[Y_{i}^{2}\right]
\]


Give an example?? 

There is a number of ways to correct this. Scale all the coefficients
so that they have the same variance:
\[
\hat{\Sigma}_{ij}=\begin{cases}
\alpha_{ij}\mathbb{E}_{i\cap j}\left[Y_{i}Y_{j}\right]-\mathbb{E}_{i}\left[Y_{i}\right]\mathbb{E}_{j}\left[Y_{j}\right] & \text{if }N_{ij}>0\\
0 & \text{otherwise}
\end{cases}
\]
\[
\alpha_{ij}=\sqrt{\frac{\mathbb{E}_{i}\left[Y_{i}^{2}\right]\mathbb{E}_{j}\left[Y_{j}^{2}\right]}{\mathbb{E}_{i\cap j}\left[Y_{i}^{2}\right]\mathbb{E}_{i\cap j}\left[Y_{j}^{2}\right]}}
\]



\subsection{Learning}


\subsection{Inference
\[
\mathbf{e}\left(\mathbf{s}\right)\in\left\{ 0,1\right\} ^{n}=\sum_{i}\mathbf{e}_{\beta\left(l_{i},s_{i}\right)}
\]
}

The inference works this way:
\[
Y_{\left(p\right)}=\sum_{\mathbf{s}}\mathbf{1}_{\mathbf{s}}\left(s\right)\cdot\mathbf{e}\left(\mathbf{s}\right)^{T}Y
\]
\[
s\sim\text{HMM}\left(p\right)
\]
\[
f\left(t\right)=\sum_{s_{1}\in S_{l_{1}}}\cdots\sum_{s_{M}\in S_{l_{M}}}\pi\left(\mathbf{s}\right)\pi_{Y_{\left(\mathbf{s}\right)}}\left(t\right)
\]
\[
Y_{|s}=\mathbf{e}\left(\mathbf{s}\right)^{T}Y=\sum_{i}Y_{l_{i},s_{i}}\sim\mathcal{N}\left(\mathbf{e}\left(\mathbf{s}\right)^{T}\mu,\mathbf{e}\left(\mathbf{s}\right)^{T}\Sigma\mathbf{e}\left(\mathbf{s}\right)\right)
\]
\[
\mathbf{e}\left(\mathbf{s}\right)^{T}\Sigma\mathbf{e}\left(\mathbf{s}\right)\approx\left\Vert \sum_{i}Q_{\beta\left(l_{i},s_{i}\right)}\right\Vert ^{2}
\]


Approximation of the covariance matrix

We need to solve two problems:

Compute the variances of each sequence of variables:
\[
\mathbf{e}\left(\mathbf{s}\right)^{T}\Sigma\mathbf{e}\left(\mathbf{s}\right)
\]
with $\mathbf{s}$ being a valid sequence of variables in the graph
of variables.

Compute the elements of the covariance matrix that correspond to the
non-zeros of the precision matrix:
\[
\Sigma_{ij}\,\text{for }\left(i,j\right)\,\in??
\]


We propose to solve both problems using random projections. These
problems are quite similar since:
\[
\Sigma_{ij}=\frac{1}{2}\left(\left\Vert \mathbf{e}_{i}\right\Vert _{L}^{2}+\left\Vert \mathbf{e}_{j}\right\Vert _{L}^{2}-\left\Vert \mathbf{e}_{i}+\mathbf{e}_{j}\right\Vert _{L}^{2}\right)
\]


The key insight is to recognize that $x^{T}\Sigma x$ is the squared
norm of $x$ for a certain norm function. Using the Jonhson-Lindenstrauss
theorem, this norm can be approximated efficiently, and in the case
of the covariance estimation, we can provide some probabilistic guarantees
about the quality of the approximation.

Lemma (adapted from Spielman)

Given fixed vectors $v_{1}\cdots v_{n}\in\mathbb{R}^{d}$ and $\epsilon>0$,
let $Q\in\mathbb{R}^{k\times d}$ be a random matrix with random Bernoulli
entries $\pm1/\sqrt{k}$ and with $k\geq24\epsilon^{-2}\log n$. Then
with probability at least $1-1/n$:
\[
\left(1-\epsilon\right)\left\Vert v_{i}\right\Vert ^{2}\leq\left\Vert Qv_{i}\right\Vert ^{2}\leq\left(1+\epsilon\right)\left\Vert v_{i}\right\Vert ^{2}
\]


Consider the Cholesky factorization of the precision matrix:
\[
S=LL^{T}
\]
with $L$ real and upper-triangular. Consider a vector $x\in$Then:
\begin{eqnarray*}
x^{T}\Sigma x & = & x^{T}L^{-T}L^{-1}x\\
 & = & \left\Vert L^{-1}x\right\Vert ^{2}\\
 & = & \left\Vert x\right\Vert _{L}^{2}
\end{eqnarray*}
\[
x^{T}\Sigma x=x^{T}L^{-T}L^{-1}x=\left\Vert L^{-1}x\right\Vert ^{2}
\]


The fundamental request is to compute the variance along a series
of states

In particular:
\[
\Sigma_{ii}=\mathbf{e}_{i}^{T}\Sigma\mathbf{e}_{i}=\left\Vert \mathbf{e}_{i}\right\Vert _{L}^{2}
\]
\[
R=L^{-1}Q
\]
\[
\nabla_{uv}=\hat{\Sigma}_{uv}-R_{u}^{T}R_{v}
\]


==> pipeline.tex <==
%!TEX root = article.tex
% \begin{figure}
% \centering
% \includegraphics[width=\columnwidth]{x.png}
% \caption{A sample black and white graphic (.eps format)
% that has been resized with the command.}
% \end{figure}

\pacomment{Pretty much this entire section seems redundant and could
  be cut / few non-redundant points could be made in intro?}

\tjhcomment{Not sure about the goal of this whole section, it seems
to be very high level and may go in the intro}

Here we give an overview of the pipeline for estimating travel time
distributions before giving details on the components in subsequent
sections.


\subsection{Processing GPS traces}

% (fold)
\label{sub:processing_gps_traces}

A raw GPS trace can be seen as a sequence of coordinate locations
with timestamps. A first step we take in extracting travel time information
from a trace is matching the coordinates to points along a particular
path. Each sample coordinate is now mapped to a link and an offset
distance from the beginning of the link. An efficient algorithm was
developed for this path-matching and path-inference step and is discussed
in~\cite{hunter11pif}. We do not detail this algorithm here.

We then make the observation that the travel time a vehicle experiences
on a particular link is highly correlated with the number of red lights
experienced (or more generally, the number of stops experienced).
Therefore, we wish to learn when a vehicle comes to a stop along a
traveled route. We do this by mapping the path-matched trace to a
set of stopping times and locations along the path. This algorithm
is called the \stopgo{} and is detailed in Section~\ref{sec:stop-and-go}.

% subsection processing_gps_traces (end)    



\subsection{Learning state transitions for neighboring links on a path}

% (fold)
\label{sub:learning_state_transition_}

\begin{figure}
\centering \label{fig:mode-histograms}
\includegraphics[width=0.8\columnwidth]{figs-plots/example_bimodal_link}
\vspace*{-.6cm}
\caption{Histograms for observed travel times on a number of links. Observations
tend to cluster around a discrete number of modes.}
\end{figure}


\tjhcomment{could be shortened, given what we say in intro}

When observing empirical link travel time data, multiple \emph{modes}
tend to appear. Examples of these modes to are shown in Figure~\ref{fig:mode-histograms}.
We hypothesize that a particular observation's mode on a link is determined
by the number of stops experienced, which we denote as the \emph{state}.
Thus, the output of the \stopgo{} will be directly used to label
the states of all links traversed by a vehicle path observation.

\jdrcomment{is there a need to standardize route vs. path? Should
we use just one word for the entire article?}

For a single path observation, we model the state transitions as a
Markov model, i.e. the state of the next link is a function of only
the state of the previous link traversed along the path. Running all
input GPS traces through the \stopgo produces a set of labeled data
to train the Markov model. The training step outputs a state transition
matrix, $\TMM$, and initial probability vector, $\initProbMM$, which
are later used in the inference step. Section~\ref{sec:hmm} discusses
this model and the training procedure.

\tjhcomment{mu already means the mean for the gmrf}

% subsection learning_state_transition_ (end)



\subsection{Learning dependencies in link travel times}

% (fold)
\label{sub:learning_dependencies_in_link_travel_times}

While the Markov model gives transitions between states, a model is
still needed for estimating travel times for a given link and state
(number of stops experienced). Since we seek travel time distributions,
the travel time for a particular link \emph{and} state is modeled
as a Gaussian random variable. Further, using a \gmrf{} to capture
spacial dependencies, the joint probabilities are modeled as a multivariate
Gaussian.

From the output of the \stopgo, we can obtain not only states, but
also travel time observations across links with labeled states. This
data is used as input to learn the parameters of the \gmrf{}, which
include the mean vector, $\meanGMRF$, and the precision matrix, $S$.
Again, the output of this learning phase is used as input in the inference
step. Section~\ref{sec:gmrf-model} gives details on the \gmrf{}
learning step.

% subsection learning_correlated_link_travel_times (end)



\subsection{Inferring travel time distributions}

% (fold)
\label{sub:inferring_travel_time_distributions}

In our model of travel times, two distinct parts can be combined:
the whether a vehicle stops at a light or not, and how long it stays.
Indeed, some drivers may experience some longer delays (if they are
in a different lane for example)

Travel times may be correlated due to 3 reasons:

the behavior of individual drivers may be different: some car may
travel notably faster than some others, while some drivers exhibit
some more prudent attitude on the road.

As in the prediction of stops, we make the hypothesis that delays
and travel times are essentially a local phenomenon: if cars happen
to be blocked by heavy traffic, it is natural to expect that traffic
propagates through interactions with neighboring links. Thus, if a
driver experiences a slow trip on some portions of its travel, this
perturbation will probably not have dissipated when she reaches the
subsequent path. If a driver experiences a longer than usual stay
at some light due to heavy traffic, she can expect to also experience
some heavy traffic later in its trip.

In some portions of the road network and under some saturation conditions,
the vehicles may move in a coordinated fashion, in the form of platoons.
In such synchronized batches, vehicles are not free to decide their
pace at will and have to follow the average pace of their group. If
a vehicle attempts to go faster, it will inevitably hit a red light
and be joined back by the rest of its group. In this case, one may
expect some negative correlations to develop: vehicles that go faster
than the mean at some point will be slowed down, while slower vehicles
will be able to catch up with their platoons.

Traffic in a city is subject to a number of complex conditions, and
the phenomenons detailed above lead to different directions/increase
or decrease the variances/pull estimates in different directions.
As such, it is not clear that a single physical model would give some
reliable estimates. This is why we focus on a simple model that considers
travel times to follow a normal distribution (when the effect/state
of o light is already determined). The correlations between the travel
times on the links and for different states of traffic lights lead
us to consider a joint Gaussian variable.

% subsection inferring_travel_time_distributions (end)

